Age determination for 269 $Gaia$ DR2 Open Clusters

$Context$. Gaia Second Data Release provides precise astrometry and photometry for more than 1.3 billion sources. This catalog opens a new era concerning the characterization of open clusters and test stellar models, paving the way for a better understanding of the disc properties. $Aims$. The aim of the paper is to improve the knowledge of cluster parameters, using only the unprecedented quality of the Gaia photometry and astrometry. $Methods$. We make use of the membership determination based on the precise Gaia astrometry and photometry. We apply anautomated Bayesian tool, BASE-9, to fit stellar isochrones on the observed G, GBP, GRP magnitudes of the high probability member stars. $Results$. We derive parameters such as age, distance modulus and extinction for a sample of 269 open clusters, selecting only low reddening objects and discarding very young clusters, for which techniques other than isochrone-fitting are more suitable for estimating ages.

==> FINAL_TABLE_FIX_LETT.tex <==
cluster              & ra         & dec        & $\log (age)$ & $(m-M)_0$  & $A_V$      & $A_G$      & \feh      \\ \hline
Alessi5              & +160.819 & +160.819 &  7.73$^{7.74}_{7.73}$ &  7.71$^{7.72}_{7.70}$ &  0.60$^{0.61}_{0.59}$ &  0.58$^{0.60}_{0.55}$ &  -0.382\\
Alessi6              & +220.058 & +220.058 &  8.78$^{8.79}_{8.78}$ &  9.55$^{9.56}_{9.54}$ &  0.72$^{0.73}_{0.71}$ &  0.70$^{0.72}_{0.68}$ &  -0.154\\
Alessi24             & +260.764 & +260.764 &  7.95$^{7.96}_{7.92}$ &  8.30$^{8.31}_{8.29}$ &  0.34$^{0.35}_{0.33}$ &  0.33$^{0.35}_{0.30}$ &  -0.133\\
BH99                 & +159.553 & +159.553 &  7.91$^{7.92}_{7.89}$ &  8.08$^{8.10}_{8.07}$ &  0.21$^{0.22}_{0.20}$ &  0.20$^{0.22}_{0.17}$ &  0.000\\
Collinder140         & +110.882 & +110.882 &  7.47$^{7.49}_{7.45}$ &  7.81$^{7.83}_{7.78}$ &  0.11$^{0.12}_{0.10}$ &  0.10$^{0.12}_{0.08}$ &  0.010\\
Czernik27            & +105.830 & +105.830 &  9.07$^{9.07}_{9.06}$ &  12.97$^{12.98}_{12.95}$ &  0.53$^{0.55}_{0.52}$ &  0.52$^{0.56}_{0.49}$ &  -0.380\\
Harvard5             & +186.817 & +186.817 &  7.80$^{7.82}_{7.78}$ &  10.40$^{10.41}_{10.39}$ &  0.68$^{0.69}_{0.67}$ &  0.66$^{0.69}_{0.64}$ &  -0.090\\
IC1369               & +318.033 & +318.033 &  8.46$^{8.46}_{8.46}$ &  12.54$^{12.55}_{12.54}$ &  2.05$^{2.06}_{2.04}$ &  2.00$^{2.01}_{1.99}$ &  0.090\\
IC2488               & +141.857 & +141.857 &  8.21$^{8.21}_{8.20}$ &  10.63$^{10.64}_{10.62}$ &  0.70$^{0.71}_{0.70}$ &  0.69$^{0.70}_{0.67}$ &  0.080\\
IC4725               & +277.937 & +277.937 &  7.99$^{7.99}_{7.99}$ &  9.15$^{9.16}_{9.14}$ &  1.08$^{1.09}_{1.08}$ &  1.06$^{1.08}_{1.05}$ &  0.000\\
King6                &  +51.982 &  +51.982 &  8.58$^{8.58}_{8.58}$ &  9.54$^{9.55}_{9.54}$ &  1.10$^{1.11}_{1.10}$ &  1.08$^{1.10}_{1.06}$ &  0.460\\
Lynga1               & +209.994 & +209.994 &  7.93$^{8.04}_{7.79}$ &  11.76$^{11.79}_{11.74}$ &  1.51$^{1.53}_{1.48}$ &  1.47$^{1.52}_{1.42}$ &  0.020\\
NGC0381              &  +17.094 &  +17.094 &  8.71$^{8.74}_{8.68}$ &  10.53$^{10.54}_{10.52}$ &  1.04$^{1.05}_{1.03}$ &  1.02$^{1.05}_{0.99}$ &  0.070\\
NGC2215              &  +95.199 &  +95.199 &  8.80$^{8.82}_{8.77}$ &  9.84$^{9.86}_{9.83}$ &  0.86$^{0.87}_{0.85}$ &  0.84$^{0.88}_{0.82}$ &  -0.400\\
NGC2281              & +102.091 & +102.091 &  8.78$^{8.80}_{8.78}$ &  8.46$^{8.47}_{8.46}$ &  0.13$^{0.14}_{0.12}$ &  0.13$^{0.16}_{0.12}$ &  0.130\\
NGC2343              & +107.029 & +107.029 &  7.93$^{7.94}_{7.92}$ &  10.07$^{10.08}_{10.06}$ &  0.50$^{0.51}_{0.48}$ &  0.48$^{0.51}_{0.46}$ &  0.030\\
NGC2422              & +114.147 & +114.147 &  8.11$^{8.11}_{8.10}$ &  8.25$^{8.26}_{8.25}$ &  0.20$^{0.21}_{0.19}$ &  0.27$^{0.27}_{0.27}$ &  0.090\\
NGC2546              & +123.082 & +123.082 &  7.96$^{7.98}_{7.96}$ &  9.82$^{9.83}_{9.81}$ &  0.46$^{0.47}_{0.45}$ &  0.45$^{0.47}_{0.43}$ &  0.010\\
NGC2658              & +130.868 & +130.868 &  8.70$^{8.71}_{8.70}$ &  12.87$^{12.88}_{12.86}$ &  0.70$^{0.71}_{0.70}$ &  0.69$^{0.70}_{0.68}$ &  -0.010\\
NGC2818              & +139.044 & +139.044 &  8.96$^{8.96}_{8.96}$ &  12.49$^{12.50}_{12.48}$ &  0.60$^{0.60}_{0.60}$ &  0.59$^{0.61}_{0.57}$ &  -0.170\\
NGC2972              & +145.058 & +145.058 &  8.64$^{8.66}_{8.63}$ &  11.41$^{11.42}_{11.39}$ &  1.20$^{1.21}_{1.18}$ &  1.17$^{1.20}_{1.14}$ &  -0.090\\
NGC3228              & +155.378 & +155.378 &  7.42$^{7.42}_{7.42}$ &  8.36$^{8.36}_{8.34}$ &  0.13$^{0.14}_{0.12}$ &  0.13$^{0.15}_{0.11}$ &  0.010\\
NGC4609              & +190.582 & +190.582 &  7.52$^{7.53}_{7.52}$ &  10.88$^{10.89}_{10.87}$ &  1.07$^{1.08}_{1.06}$ &  1.04$^{1.06}_{1.02}$ &  0.050\\
NGC5138              & +201.829 & +201.829 &  7.64$^{7.64}_{7.63}$ &  11.50$^{11.51}_{11.48}$ &  0.76$^{0.76}_{0.75}$ &  0.74$^{0.76}_{0.72}$ &  0.120\\
NGC5281              & +206.614 & +206.614 &  7.65$^{7.67}_{7.64}$ &  10.94$^{10.95}_{10.92}$ &  0.82$^{0.83}_{0.81}$ &  0.80$^{0.82}_{0.77}$ &  -0.020\\
NGC5316              & +208.516 & +208.516 &  8.18$^{8.19}_{8.18}$ &  10.79$^{10.80}_{10.78}$ &  0.77$^{0.78}_{0.76}$ &  0.75$^{0.77}_{0.74}$ &  0.130\\
NGC5460              & +211.847 & +211.847 &  8.09$^{8.15}_{8.06}$ &  9.25$^{9.26}_{9.24}$ &  0.33$^{0.34}_{0.32}$ &  0.32$^{0.34}_{0.30}$ &  0.030\\
NGC5617              & +217.452 & +217.452 &  8.14$^{8.14}_{8.14}$ &  11.66$^{11.66}_{11.65}$ &  1.59$^{1.60}_{1.59}$ &  1.55$^{1.56}_{1.54}$ &  -0.180\\
NGC6025              & +240.779 & +240.779 &  8.10$^{8.10}_{8.10}$ &  9.47$^{9.47}_{9.46}$ &  0.40$^{0.41}_{0.39}$ &  0.51$^{0.51}_{0.51}$ &  0.190\\
NGC6204              & +251.538 & +251.538 &  7.58$^{7.58}_{7.57}$ &  10.50$^{10.51}_{10.49}$ &  1.29$^{1.30}_{1.28}$ &  1.26$^{1.28}_{1.23}$ &  0.020\\
NGC6208              & +252.336 & +252.336 &  9.22$^{9.22}_{9.22}$ &  10.35$^{10.35}_{10.34}$ &  0.63$^{0.64}_{0.63}$ &  0.62$^{0.63}_{0.60}$ &  -0.010\\
NGC6716              & +283.616 & +283.616 &  7.93$^{7.94}_{7.92}$ &  9.12$^{9.13}_{9.10}$ &  0.71$^{0.72}_{0.69}$ &  0.69$^{0.72}_{0.66}$ &  -0.310\\
NGC6830              & +297.718 & +297.718 &  8.01$^{8.03}_{8.00}$ &  11.87$^{11.88}_{11.86}$ &  1.52$^{1.53}_{1.51}$ &  1.48$^{1.50}_{1.45}$ &  0.220\\
NGC6866              & +300.983 & +300.983 &  8.89$^{8.89}_{8.88}$ &  10.64$^{10.65}_{10.63}$ &  0.40$^{0.41}_{0.39}$ &  0.39$^{0.44}_{0.37}$ &  -0.013\\
NGC6940              & +308.626 & +308.626 &  9.01$^{9.01}_{9.01}$ &  10.07$^{10.08}_{10.06}$ &  0.45$^{0.46}_{0.45}$ &  0.44$^{0.47}_{0.01}$ &  0.150\\
NGC7092              & +322.889 & +322.889 &  8.49$^{8.52}_{8.46}$ &  7.22$^{7.23}_{7.21}$ &  0.05$^{0.06}_{0.04}$ &  0.03$^{0.03}_{0.03}$ &  0.000\\
NGC7209              & +331.224 & +331.224 &  8.53$^{8.53}_{8.53}$ &  10.33$^{10.34}_{10.33}$ &  0.55$^{0.55}_{0.54}$ &  0.53$^{0.55}_{0.52}$ &  0.070\\
NGC7243              & +333.788 & +333.788 &  8.01$^{8.01}_{8.00}$ &  9.74$^{9.75}_{9.74}$ &  0.57$^{0.58}_{0.57}$ &  0.56$^{0.58}_{0.54}$ &  0.030\\
NGC7296              & +337.000 & +337.000 &  7.92$^{7.93}_{7.92}$ &  12.07$^{12.08}_{12.06}$ &  0.71$^{0.73}_{0.70}$ &  0.69$^{0.72}_{0.67}$ &  -0.020\\
Pismis4              & +128.790 & +128.790 &  7.91$^{7.91}_{7.90}$ &  9.11$^{9.12}_{9.10}$ &  0.09$^{0.10}_{0.09}$ &  0.09$^{0.10}_{0.08}$ &  -0.200\\
Ruprecht1            &  +99.084 &  +99.084 &  8.48$^{8.49}_{8.47}$ &  10.78$^{10.79}_{10.77}$ &  0.70$^{0.71}_{0.70}$ &  0.68$^{0.70}_{0.66}$ &  -0.250\\
Ruprecht93           & +166.037 & +166.037 &  8.54$^{8.55}_{8.52}$ &  11.68$^{11.69}_{11.67}$ &  0.64$^{0.64}_{0.63}$ &  0.63$^{0.65}_{0.60}$ &  0.153\\
Ruprecht115          & +243.215 & +243.215 &  8.40$^{8.40}_{8.40}$ &  11.88$^{11.90}_{11.87}$ &  2.34$^{2.35}_{2.33}$ &  2.26$^{2.30}_{2.23}$ &  0.010\\
Ruprecht151          & +115.315 & +115.315 &  8.61$^{8.62}_{8.60}$ &  10.36$^{10.38}_{10.34}$ &  0.59$^{0.61}_{0.57}$ &  0.57$^{0.61}_{0.53}$ &  -0.102\\
Trumpler10           & +131.943 & +131.943 &  7.74$^{7.75}_{7.74}$ &  7.81$^{7.82}_{7.80}$ &  0.14$^{0.14}_{0.13}$ &  0.17$^{0.17}_{0.17}$ &  -0.120\\
Trumpler22           & +217.783 & +217.783 &  7.38$^{7.39}_{7.38}$ &  11.87$^{11.88}_{11.86}$ &  1.83$^{1.84}_{1.83}$ &  1.79$^{1.81}_{1.77}$ &  -0.170\\
